On the convergence rate of noisy Bayesian Optimization with Expected Improvement

Expected improvement (EI) is one of the most widely used acquisition functions in Bayesian optimization (BO). Despite its proven success in applications for decades, important open questions remain on the theoretical convergence behaviors and rates for EI. In this paper, we contribute to the convergence theory of EI in three novel and critical areas. First, we consider objective functions that fit under the Gaussian process (GP) prior assumption, whereas existing works mostly focus on functions in the reproducing kernel Hilbert space (RKHS). Second, we establish for the first time the asymptotic error bound and its corresponding rate for GP-EI with noisy observations under the GP prior assumption. Third, by investigating the exploration and exploitation properties of the non-convex EI function, we establish improved error bounds of GP-EI for both the noise-free and noisy cases.

==> Sections/Cumulative.tex <==
\section{Cumulative regret bound}\label{se:regret}
In this section, we consider the cumulative regret of BO-EI under the GP prior assumption.
The instantaneous regret $r_t$ is often defined as $f(\xbm_{t+1})-f(\xbm^*)$, \textit{e.g.}, for UCB~\cite{srinivas2009gaussian}.
Since it measures the loss in reward function, we propose the following novel definition  
 \begin{equation} \label{eqn:cumu-error}
 \centering
  \begin{aligned}
       r_t = I_t(\xbm^*) - I_t(\xbm_{t+1}) = \max\{y^+_{t}-f(\xbm^*),0\}-\max\{y^+_{t}-f(\xbm_{t+1}),0\}\geq 0.
  \end{aligned}
\end{equation}
   We note that $r_t$ in~\eqref{eqn:cumu-error} is non-negative since $f(\xbm^*)\leq f(\xbm_{t+1})$.
   The main difference in~\eqref{eqn:cumu-error} is that instead of $f$, we use the improvement function $I_t$.
   Given that EI is constructed upon the improvement function, $I_t$ is a reasonable measure of reward.
Further, the observation $y^+_t$ and improvement function $I_t$  are fully incorporated in the BO-EI algorithm to determine the next best sample.
  Therefore, the adoption of $I_t$ is a natural extension of the algorithm itself. 
  From the theory perspective, our definition allows us to overcome the difficulty in providing a lower bound for $y_t^+-f(\xbm_{t+1})$ when $y_t^+-f(\xbm_{t+1})<0$, as its contribution to $r_t$ measures $0$. 
  This is an important step that previous papers dealt with by requiring additional modification of EI. 
  For example, in~\cite{nguyen17a}, the authors used a stopping criterion to achieve a lower bound. Others have resorted to modification of the BO-EI algorithm with new algorithmic parameters~\cite{tran2022regret}. 

To obtain a desirable cumulative regret bound, we first need to expand on the results in section~\ref{se:analysis} to include all $\xbm\in C$ and $t\in \Nbb$ when possible.
In addition, we distinguish between two cases of $C$: we assume first a discrete $C$ and later expands it to be compact, as in~\cite{srinivas2009gaussian}. 
\subsection{Finite discrete prior}\label{se:regret-discrete}
We first assume that $f$ is from a zero mean GP prior and $C$ is discrete, \textit{i.e.}, Assumption~\ref{assp:gp} and~\ref{assp:discrete}.
We first extend Lemma~\ref{lem:fmu} to all $C$ and $t$.
\begin{lemma}\label{lem:discrete-fmu}
Given $\delta\in(0,1)$, let  $\beta_t \geq 2\log(|C|\pi_t /\delta)$, where $\pi_t$ satisfies $\sum_{t=1}^{\infty} \frac{1}{\pi_t}=1,\pi_t>0$. Then,  $\forall x\in C$, $t\geq 1$,   
\begin{equation} \label{eqn:discrete-fmu-1}
 \centering
  \begin{aligned}
     |f(\xbm) - \mu_{t}(\xbm)  | \leq \beta_t^{1/2} \sigma_{t}(\xbm), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}
The proof of Lemma~\ref{lem:discrete-fmu} can be found in Lemma 5.1 in~\cite{srinivas2009gaussian} and is similar to that of Lemma~\ref{lem:fmu-alpha}. The difference is the use of union bound to include all $\xbm\in C$ and $t\in\Nbb$. 
As a result, $\beta_t\to\infty$ as $t\to\infty$.
Similarly, we can extend Lemma~\ref{lem:fmu-alpha}.
\begin{lemma}\label{lem:discrete-fmu-alpha}
Given $\delta\in(0,1)$, let  $\beta_t \geq 2\sigma_t^{2(1-\alpha)}(\xbm)\log(|C|\pi_t /\delta)$, where $\pi_t$ satisfies $\sum_{t=1}^{\infty} \frac{1}{\pi_t}=1,\pi_t>0$. Then,  $\forall x\in C$, $t\geq 1$,   
\begin{equation} \label{eqn:discrete-fmu-alpha-1}
 \centering
  \begin{aligned}
     |f(\xbm) - \mu_{t}(\xbm)  | \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}
The upper bounds in~\eqref{eqn:discrete-fmu-1} and~\eqref{eqn:discrete-fmu-alpha-1} are the same if $\beta_t$ is chosen with equality. The difference appears when applied to algorithm where $\alpha>1$. 
Next, we state the extension of Lemma~\ref{lem:IEIbound}.
\begin{lemma}\label{lem:discrete-bound}
Given $\delta\in(0,1)$, let $\beta_t \geq \max\{1,c_{\beta}^{-1}\log(|C|c_{\alpha}\sigma_t^{\alpha-1}(\xbm)\pi_t /\delta)\}$, where $\sum_{t=1}^{\infty}\pi_t=1$, $c_{\alpha} \geq 1.09$ and $c_{\beta}=0.227( \sigma_t^{\alpha-1}(\xbm))^2+0.2$. Then,  $\forall x\in C$, $t\geq 1$,   
\begin{equation} \label{eqn:discrete-bound-1}
 \centering
  \begin{aligned}
     |I_t(\xbm) - EI_{t}(\xbm,\alpha)  | \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}
\begin{proof}
  From Lemma~\ref{lem:IEIbound}, at $t$ and $\xbm$, we have~\eqref{eqn:IEI-bound-pf-15}. 
Substituting $w$ with $\beta_t^{1/2}$, the union bound of all $x\in C$ is 
  \begin{equation} \label{eqn:discrete-bound-pf-1}
  \centering
  \begin{aligned}
       P\left\{ \bigcup_{x\in C} \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| > \beta_t^{1/2} \right\}\leq& 
       \sum_{x\in C} P\left\{ \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| > \beta_t^{1/2} \right\}  \\
       \leq& |C| c_{\alpha} \sigma_t^{\alpha-1}(\xbm) e^{-0.227\sigma_t^{2(\alpha-1)}(\xbm) \beta_t}e^{-0.2\beta_t},
  \end{aligned}
\end{equation}
where $c_{\alpha}=1.09$.
 Next, we apply the union bound over all iterations $t$ to get
   \begin{equation} \label{eqn:discrete-bound-pf-2}
  \centering
  \begin{aligned}
       P\left\{ \bigcup_{t=1}^{\infty} \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| > \beta_t^{1/2}, \forall x\in C \right\} 
       \leq& \sum_{t=1}^{\infty} P\left\{ \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| > \beta_t^{1/2}, \forall x\in C \right\} \\ 
       \leq& \sum_{t=1}^{\infty} |C| c_{\alpha} \sigma_t^{\alpha-1}(\xbm) e^{-0.227\sigma_t^{2(\alpha-1)}(\xbm) \beta_t}e^{-0.2\beta_t}.
  \end{aligned}
\end{equation}
 Let 
   \begin{equation} \label{eqn:discrete-bound-pf-3}
  \centering
  \begin{aligned}
     \sum_{t=1}^{\infty} |C| c_{\alpha} \sigma_t^{-1+\alpha}(\xbm) e^{-0.227\sigma_t^{-2(1-\alpha)}(\xbm) \beta_t}e^{-0.2\beta_t} = \delta. 
  \end{aligned}
\end{equation}
Choose $\pi_t$ so that $\sum_{t=1}^{\infty} \frac{1}{\pi_t}=1$.
   Let
   \begin{equation} \label{eqn:discrete-bound-pf-4}
  \centering
  \begin{aligned}
     |C| c_{\alpha} \sigma_t^{-1+\alpha}(\xbm) e^{-0.227\sigma_t^{-2(1-\alpha)}(\xbm) \beta_t}e^{-0.2\beta_t} = \frac{\delta}{\pi_t}. 
  \end{aligned}
\end{equation}
  Taking the logarithm of~\eqref{eqn:discrete-bound-pf-4} gives us the $\beta_t$ in the condition of the lemma.
  Then, we have  
   \begin{equation} \label{eqn:discrete-bound-pf-5}
  \centering
  \begin{aligned}
       P\left\{ \bigcup_{t=1}^{\infty} \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| > \beta_t^{1/2}, \forall x\in C \right\} 
       \leq \delta.
  \end{aligned}
\end{equation}
  Therefore,  
   \begin{equation} \label{eqn:discrete-bound-pf-6}
  \centering
  \begin{aligned}
       P\left\{ \left|\frac{I_t(\xbm) - EI_{t}(\xbm,\alpha)}{\sigma_{t}^{\alpha}(\xbm)}\right| < \beta_t^{1/2}  \right\} \geq 1-\delta. 
  \end{aligned}
\end{equation}
\end{proof}
From here on, for simplicity of presentation, we choose $\pi_t=\frac{\pi^2t^2}{6}$.
\begin{remark}\label{remark:betat}
From Lemma~\ref{lem:log-1}, $\beta_t$ in Lemma~\ref{lem:discrete-bound} can be viewed as $h(x)$ with $a=0.227$, $b=0.2$, $c=1.09|C|\sigma_t^{\alpha-1}(\xbm)\frac{\pi^2t^2}{6}\geq 1.79|C|t^2 $, $d=\delta$.
  The conditions in Lemma~\ref{lem:log-1} is satisfied for $t\geq 2$ or $\delta\leq 0.698$. Therefore, $c_{\beta}^{-1}(\xbm)\log(|C|c_{\alpha}\sigma_t^{\alpha-1}(\xbm)\pi_t /\delta)\leq \frac{1}{0.427}\log(|C|c_{\alpha}\pi_t/\delta)$ if $\delta\leq 0.698$.
\end{remark}
The following two Lemmas are well-established results from~\cite{srinivas2009gaussian} on the information gain and variances.
\begin{lemma}\label{lem:infogain}
   Given observations  $\ybm_T=[y_1,\dots,y_T]$ and function values $\fbm_T=[f(\xbm_1),\dots,f(\xbm_T)]$ at the set of points $A_t=\{\xbm_1,\dots,\xbm_T\}$, the information gain is 
    \begin{equation} \label{eqn:info-1}
  \centering
  \begin{aligned}
       I(\ybm_T;\fbm_T) = \frac{1}{2} \sum_{t=1}^T \log(1+\sigma^{-2}\sigma_{t-1}^2(\xbm_t)). 
  \end{aligned}
\end{equation}
\end{lemma}
As in~\cite{srinivas2009gaussian,bull2011convergence},  we use  $\gamma_T$ to bound the sum of variance at $A_t$.
\begin{lemma}\label{lem:variancebound}
 The sum of posterior variance functions $\sigma_{t}(\xbm)$ satisfies
 \begin{equation} \label{eqn:var-1}
  \centering
  \begin{aligned}
    \sum_{t=1}^T  \sigma_{t-1}^2(\xbm) \leq \frac{1}{4}C_{\gamma} \gamma_T, 
  \end{aligned}
\end{equation}
 where $C_{\gamma} = 8/log(1+\sigma^{-2})$.
\end{lemma}
%\begin{proof}
%   The logarithm function satisfies $\frac{x}{\log(1+x)}\geq 1$. 
%   Given the assumption $\sigma_{t-1}(\xbm)\leq k(\xbm,\xbm)\leq 1$, one can write $\sigma^{-2} \sigma_{t-1}^2(\xbm)\leq \sigma^{-2}$. 
%   Consequently,  
% \begin{equation} \label{eqn:sqrreg-2}
%  \centering
%  \begin{aligned}
 %     \frac{\sigma^{-2} \sigma_{t-1}^2(\xbm)}{\log(1+\sigma^{-2} \sigma_{t-1}^2(\xbm))}\leq \frac{\sigma^{-2}}{\log(1+\sigma^{-2})}. 
%  \end{aligned}
%\end{equation}
%  Using Lemma~\ref{lem:infogain} and the definition of $\gamma_T$, 
% \begin{equation} \label{eqn:sqrreg-3}
%  \centering
%  \begin{aligned}
%    \sum_{t=1}^T  \sigma_{t-1}^2(\xbm) \leq  \sum_{t=1}^T\frac{\log(1+\sigma^{-2} \sigma_{t-1}(\xbm))^2}{\log(1+\sigma^{-2})}=&
%              \frac{2}{\log(1+\sigma^{-2})}\sum_{t=1}^T \frac{1}{2}\log(1+\sigma^{-2} \sigma_{t-1}^2(\xbm)) \\
%              \leq&  \frac{2}{\log(1+\sigma^{-2})}\gamma_T = \frac{1}{4} C_{\gamma} \gamma_T.\\
%  \end{aligned}
%\end{equation}
%\end{proof}
The conditions for regret bound can now be established.
\begin{theorem}\label{theorem:EI-regret}
   Given $\delta\in(0,0.698)$, let $\beta_t=\max\{1, c_{\beta}^{-1} \log (2|C|c_{\alpha}\pi_t/\delta)\}$, where $c_{\beta}=0.427,c_{\alpha}=1.09$, and $\pi_t=\frac{\pi^2t^2}{6}$.
   Running the BO-EI algorithm with GP prior $(0,k(\xbm,\xbm'))$ leads to the regret bound 
      \begin{equation} \label{eqn:discrete-regret-1}
  \centering
  \begin{aligned}
      R_T \leq 0.4\left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}} + \frac{1}{2} (C_{\gamma}T\beta_T\gamma_T)^{1/2}+\beta_T^{1/2} \sum_{t=1}^{T} \sigma_{t}^{\alpha}(\xbm^*).
   \end{aligned}
  \end{equation} 
  with probability $\geq 1-\delta$.
\end{theorem}
\begin{proof}
   We first note that due to Remark~\ref{remark:betat}, the $\beta_t$ satisfies  Lemma~\ref{lem:discrete-bound} and Lemma~\ref{lem:discrete-fmu} with $\delta/2$. That is~\eqref{eqn:discrete-bound-1} and~\eqref{eqn:discrete-fmu-1} are satisfied with probability $\geq 1-\delta/2$ each. 
  If $y^+_{t}-f(\xbm_{t+1})\leq 0$, with probability $\geq 1-\delta$, we have
  \begin{equation} \label{eqn:EI-insregret-pf-1}
  \centering
  \begin{aligned}
          r_t  \leq& y^+_{t}-f(\xbm^*)\leq I_t(\xbm^*,\alpha)\leq EI_{t}(\xbm^*,\alpha) + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*) 
                   \leq EI_{t}(\xbm_{t+1},\alpha) + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)\\
                =& (y^+_{t}-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))  + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)\\
                \leq& (y^+_{t}-f(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))+ f(\xbm_{t+1})-\mu_t(\xbm_{t+1})+0.4\sigma_{t}^{\alpha}(\xbm_{t+1})  + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)\\
                \leq& \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+0.4\sigma_{t}^{\alpha}(\xbm_{t+1}) + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*).\\
  \end{aligned}
  \end{equation}
  The third inequality on the first line of~\eqref{eqn:EI-insregret-pf-1} uses Lemma~\ref{lem:discrete-bound} with $\delta/2$. The third line uses $\phi(\cdot)<0.4$ and the fourth line uses $y^+_{t}-f(\xbm_{t+1})\leq 0$ and Lemma~\ref{lem:discrete-fmu} with $\delta/2$.
  If $y^+_{t}-f(\xbm_{t+1})> 0$, using Lemma~\ref{lem:discrete-bound} with $\delta/2$, with probability $\geq 1-\delta/2$,
  \begin{equation} \label{eqn:EI-insregret-pf-2}
  \centering
  \begin{aligned}
          r_t =& f(\xbm_{t+1})-f(\xbm^*) =  f(\xbm_{t+1})-y^+_{t}+ y^+_{t}-f(\xbm^*)\\
              \leq& f(\xbm_{t+1})-y^+_{t}+EI_{t}(\xbm_{t+1},\alpha) + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)\\
                =& f(\xbm_{t+1})-y^+_{t}+(y^+_{t}-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))  \\
                 &+ \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*).\\
  \end{aligned}
  \end{equation}
  Applying Lemma~\ref{lem:discrete-fmu} with $\delta/2$ to~\eqref{eqn:EI-insregret-pf-2} and $\Phi(\cdot)\leq 1$, we have
  \begin{equation} \label{eqn:EI-insregret-pf-3}
  \centering
  \begin{aligned}
         r_t \leq& f(\xbm_{t+1})-y^+_{t}+y^+_{t}-f(\xbm_{t+1})+(f(\xbm_{t+1})-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))+0.4\sigma_{t}^{\alpha}(\xbm_{t})  \\
           &+ \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)  \leq \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+0.4\sigma_{t}^{\alpha}(\xbm_{t+1}) + \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*),\\
  \end{aligned}
  \end{equation}
  with probability $\geq 1-\delta$.
  Combining~\eqref{eqn:EI-insregret-pf-2} and~\eqref{eqn:EI-insregret-pf-3}, the cumulative regret $R_T$ can be written as 
   \begin{equation} \label{eqn:EI-insregret-pf-4}
  \centering
  \begin{aligned}
      R_T = \sum_{t=1}^{T} r_t \leq  \beta_T^{1/2}\sum_{t=1}^{T} \sigma_{t}(\xbm_{t+1}) +0.4\sum_{t=1}^{T}\sigma_{t}^{\alpha}(\xbm_{t+1}) +\beta_T^{1/2} \sum_{t=1}^{T} \sigma_{t}^{\alpha}(\xbm^*).
   \end{aligned}
  \end{equation}
   From Hölder's inequality, a generalization of the Cauchy-Schwarz inequality, and Lemma~\ref{lem:variancebound}, 
   \begin{equation} \label{eqn:EI-insregret-pf-5}
    \centering
   \begin{aligned}
      \sum_{t=1}^{T}  \sigma_{t}^{\alpha}(\xbm_{t+1}) \leq& \left(\sum_{t=1}^{T} [\sigma_{t}^{\alpha}(\xbm_{t+1})]^{\frac{2}{\alpha}}\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}}  = \left(\sum_{t=1}^{T} \sigma_{t}^{2}(\xbm_{t+1})\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}}\\
    \leq& \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}},
   \end{aligned}
  \end{equation}
  Similarly, 
   \begin{equation} \label{eqn:EI-insregret-pf-6}
    \centering
   \begin{aligned}
       \sum_{t=1}^{T} \sigma_{t}(\xbm_{t+1}) \leq \frac{1}{2} (C_{\gamma} T \gamma_T)^{1/2}. 
   \end{aligned}
  \end{equation}
  Applying~\eqref{eqn:EI-insregret-pf-5} and~\eqref{eqn:EI-insregret-pf-6} to~\eqref{eqn:EI-insregret-pf-4} leads to~\eqref{eqn:discrete-regret-1} with probability $\geq 1-\delta$.
\end{proof}
\begin{remark}
   If $\sum_{t=1}^T \beta_t\sigma_t(\xbm^*) = o(T)$ for a particularly run using common kernels, \textit{e.g.}, squared exponential kernels, then BO-EI is a no-regret algorithm. 
\end{remark}
\subsection{Compact Gaussian prior}\label{se:compact}
In this section, 
$C$ is generalized to Assumption~\ref{assp:constraint}.
In~\cite{srinivas2009gaussian}, the authors assumed a lower bound on the derivatives of the kernel functions $k(\xbm,\xbm')$ with high probability. 
 That is there exist constants $a,b>0$ such that the bounded kernel $k(\xbm,\xbm')\leq 1$ satisfies 
 \begin{equation} \label{eqn:kbounded-1}
  \centering
  \begin{aligned}
     P\{\sup_{x\in C} |\partial f/\partial x_j| > L \} \leq a e^{-(\frac{L}{b})^2},
  \end{aligned}
\end{equation}
While this assumption is only used to derive a Lipschitz continuous $f$ with a high probability, the statement implies that $k(\xbm,\xbm')$ is differentiable.  
In~\cite{lederer2019uniform}, the authors assumed Lipschitz kernels that are again defined with the partial derivatives of the kernels. The author further assumed Lipschitz continuity of $f$.
From a nonsmooth optimization perspective, Lipschitz continuity is a more general condition than differentiability. Therefore, we choose to assume a Lipschitz continuous $f$ directly in Assumption~\ref{assp:gp}.  

We state an extension of Lemma~\ref{lem:fmu} using only union bound in $t\in\Nbb$ on $\xbm_t$.  
\begin{lemma}\label{lem:fmu-t}
Given $\delta\in(0,1)$, let  $\beta_t = 2\log(\pi_t /\delta)$, where $\pi_t$ satisfies $\sum_{t=1}^{\infty} \frac{1}{\pi_t}=1,\pi_t>0$. Then,   $\forall t\geq 1$,   
\begin{equation} \label{eqn:fmu-t-1}
 \centering
  \begin{aligned}
     |f(\xbm_{t+1}) - \mu_{t}(\xbm_{t+1})  | \leq \beta_t^{1/2} \sigma_{t}(\xbm_{t+1}), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}
The proof of Lemma~\ref{lem:fmu-t} is simple and is omitted here. Readers are referred to Lemma 5.5 in~\cite{srinivas2009gaussian}.
Similarly, we state without proof the extension of Lemma~\ref{lem:fmu-alpha} to all $t\in\Nbb$.
\begin{lemma}\label{lem:fmu-t-alpha}
Given $\delta\in(0,1)$, let  $\beta_t \geq 2\sigma_t^{2(1-\alpha)}(\xbm)\log(\pi_t /\delta)$, where $\pi_t$ satisfies $\sum_{t=1}^{\infty} \frac{1}{\pi_t}=1,\pi_t>0$. Then, for $t\geq 1$,   
\begin{equation} \label{eqn:fmu-t-alpha-1}
 \centering
  \begin{aligned}
     |f(\xbm_{t+1}) - \mu_{t}(\xbm_{t+1})  | \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm_{t+1}), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}
Further, we have a similar result to Lemma~\ref{lem:discrete-bound} for $\forall t\in\Nbb$.
\begin{lemma}\label{lem:compact-bound}
Given $\delta\in(0,1)$, let $\beta_t = \max\{1,c_{\beta}^{-1}\log(c_{\alpha}\sigma_t^{\alpha-1}(\xbm)\pi_t /\delta)\}$, where $\sum_{t=1}^{\infty}\pi_t=1$, $c_{\alpha} \geq 1.09$ and $c_{\beta}=0.227( \sigma_t^{\alpha-1}(\xbm))^2+0.2$. Then,  $\forall t\geq 1$,   
\begin{equation} \label{eqn:compactbound-1}
 \centering
  \begin{aligned}
     |I_t(\xbm_{t+1}) - EI_{t}(\xbm_{t+1},\alpha)  | \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm_{t+1}), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}

Next, we consider a discretization $\Cbb(h)$ of $C$ where each $\Cbb$ comprises finite number of points in $C$. 
The size parameter $h$ is a measure of the distance between $\Cbb$ and $\forall \xbm\in C$.
The discretization aims to cover the compact set $C$ with enough points so that for any $x\in C$, the distance between $\xbm\in C$ and  $\Cbb$ can be controlled.  Denote the closest point of $\xbm$ to $\Cbb$ as 
\begin{equation} \label{eqn:close-point}
 \centering
  \begin{aligned}
 	\bar{\xbm} := \underset{\substack{\ubm}\in \Cbb}{\text{minimize}} 
	   \norm{\xbm-\ubm}. \\
  \end{aligned}
\end{equation}
The size parameter $h$ satisfies
\begin{equation} \label{eqn:compactdisc-1}
 \centering
  \begin{aligned}
     \norm{\xbm-\bar{\xbm}} \leq h, \ \forall \xbm\in C. 
  \end{aligned}
\end{equation}
The size $|\Cbb(h)|$ of the set $\Cbb(h)$ is in general reversely correlated with $h$.
Consider sequences $\{h_t\}$ and $\{\Cbb_t(h_t)\}$ where the discretization is refined as $t$ increases. 
We denote the latter as $\Cbb_t$ for simplicity.
We emphasize that the discretization does not play any role in the BO-EI algorithm. Rather, it is a analytic tool to determine $\beta_t$ and the regret bound for BO-EI.

An immediate result is a lemma for $\Cbb_t$ similar to that of Lemma~\ref{lem:discrete-bound}.
 \begin{lemma}\label{lem:discretization-bound}
Given $\delta\in(0,1)$, let  $\beta_t = \max\{1,c_{\beta}^{-1}\log(|\Cbb_t|c_{\alpha}\sigma_t^{\alpha-1}(\xbm)\pi_t /\delta)\}$, where $\sum_{t=1}^{\infty}\pi_t=1$, $c_{\alpha} \geq 1.09$ and $c_{\beta}=0.227( \sigma_t^{\alpha-1}(\xbm))^2+0.2$. Then,  $\forall x\in \Cbb_t$, $t\geq 1$,   
\begin{equation} \label{eqn:compact-bound-1}
 \centering
  \begin{aligned}
     |I_t(\xbm) - EI_{t}(\xbm,\alpha)  | \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm), 
  \end{aligned}
\end{equation}
holds with probability $\geq 1-\delta$.
\end{lemma}

Let $N_{h_t}$ be the minimum number of points needed to achieve~\eqref{eqn:compactdisc-1}. 
Given $C\subseteq [0,r]^d$, we can construct the discretization with $N_{h_t}$, which has the upper bounded 
   \begin{equation} \label{eqn:disc-size-1}
  \centering
  \begin{aligned}
     |\Cbb_t| =   N_{h_t} \leq (1+ \frac{r}{h_t})^d,
   \end{aligned}
  \end{equation}
when the points in $\Cbb_t$ are evenly spaced. 
As we will see in Lemma~\ref{lem:compact-IL}, in order to achieve no regret, we require $\sum_{t=1}^{\infty}h_t < \infty$. In this section, we adopt the common choice of $h_t$ for simplicity of presentation:
   \begin{equation} \label{eqn:ht-1}
  \centering
  \begin{aligned}
    h_t = \frac{1}{L t^{1+p}}, \ p =1.
   \end{aligned}
  \end{equation}
  Further, let the corresponding $|\Cbb_t| = (1+Lrt^2)^d$.
 
*****************************************************************************************
Now, consider the contribution of $\sum_{t=1}^T\sigma_{t-1}(\xbm_t)$ and $\sum_{t=1}^T h_t$.
For Matern kernels, trouble??
 From Lemma~\ref{}, we know $\gamma_T^{1/2}$ is the upper bound for $\sum_{t=1}^T\sigma_{t-1}(\xbm_t)$.
It is well-established that for many commonly used kernels, $\gamma_T = \mathcal{O}(\log(t))$
   \begin{equation} \label{eqn:disc-size-3}
  \centering
  \begin{aligned}
    \mathcal{O} (\log(t)^{1/2} \sigma_{t-1}(\xbm_t))=\mathcal{O} (\log(\frac{1}{h_t})^{1/2} \sigma_{t-1}(\xbm_t)) \geq  \mathcal{O}( h_t) = \mathcal{O}(\frac{1}{t^{1+p}}).
   \end{aligned}
  \end{equation}
Since $\sigma_{t}(\xbm_{t+1})$ is often assumed to be $\mathcal{O}(\log(t)^{-\frac{1}{2}-d})$.

******************************************************************************************

\begin{lemma}\label{lem:compact-IL}
Given $\delta\in(0,0.698)$, let  $\beta_t = \max\{1,c_{\beta}^{-1} \log(\pi_t c_{\alpha}/\delta)\} + c_{\beta}^{-1} d \log( 1+rt^2 L) $, where $\pi_t=\frac{\pi^2t^2}{6}$, $c_{\alpha} = 1.09$, and $c_{\beta}=0.427$. Then, with probability $\geq 1-\delta$, 
   \begin{equation} \label{eqn:compact-IL-1}
  \centering
  \begin{aligned}
          |I_t(\xbm^*) - EI_{t}(\bar{\xbm}^*_t,\alpha)| \leq \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t) + \frac{1}{t^2},
  \end{aligned}
  \end{equation}
  for $\forall t\in\Nbb$.
\end{lemma}
\begin{proof}
  From Assumption~\ref{assp:gp}, and Lemma~\ref{lem:lipschitz-cplus} in the Appendix, we know 
  \begin{equation} \label{eqn:compact-IL-pf-1}
  \centering
  \begin{aligned}
     | I_t(\xbm) - I_t(\xbm') | < L \norm{\xbm-\xbm'}.
  \end{aligned}
\end{equation}
   Applying the discretization $\Cbb_t$ and~\eqref{eqn:compactdisc-1} to~\eqref{eqn:compact-IL-pf-1}, for $\forall \xbm\in C$, we have 
    \begin{equation} \label{eqn:compact-IL-pf-2}
  \centering
  \begin{aligned}
     | I_t(\xbm_t) - I_t(\bar{\xbm}_t) | < L h_t.
  \end{aligned}
\end{equation}
   Next, choose the distance measure $h_t$ so that $L h_t  =\frac{1}{t^2}$. 
   The size of the discretization set satisfies $|\Cbb_t| \leq (1+ r t^2 L)^d$. 
   The choice of $\beta_t$ in the condition of the lemma satisfies 
    \begin{equation} \label{eqn:compact-IL-pf-3}
  \centering
  \begin{aligned}
     \beta_t \geq c_{\beta}^{-1} \log( \pi_t c_{\alpha}/\delta) + c_{\beta}^{-1}\log(|\Cbb_t|  ),
  \end{aligned}
\end{equation}
  and therefore meets the condition in Lemma~\ref{lem:discretization-bound} via Remark~\ref{remark:betat}. 
   Using~\eqref{eqn:compact-IL-pf-2} and Lemma~\ref{lem:discretization-bound}, 
   \begin{equation} \label{eqn:compact-IL-pf-4}
  \centering
  \begin{aligned}
          |I_t(\xbm^*) - EI_{t}(\bar{\xbm}^*_t,\alpha)| \leq& |I_t(\xbm^*) - I_t(\bar{\xbm}^*_t)| + |I_t(\bar{\xbm}^*_t) - EI_{t}(\bar{\xbm}^*_t,\alpha)|\\ 
        \leq& \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t) + \frac{1}{t^2},
  \end{aligned}
\end{equation}
  with probability $1-\delta$.
\end{proof}

\begin{lemma}\label{lem:compact-IL-instregret}
Given $\delta\in(0,0.698)$, let  $\beta_t = \max\{1,c_{\beta}^{-1}\log ( 2\pi_t c_{\alpha}/\delta)\} + c_{\beta}^{-1} \log(1+rt^2 L) $, where $\pi_t=\frac{\pi^2t^2}{6}$, $c_{\alpha} = 1.09$, and $c_{\beta}=0.427$. Then with probability $1-\delta$, 
   \begin{equation} \label{eqn:compact-IL-instregret-1}
  \centering
  \begin{aligned}
          r_t \leq&  \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+ \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}. 
  \end{aligned}
  \end{equation}
\end{lemma}
\begin{proof}
   Notice that the $\beta_t$ in this Lemma satisfies the conditions in both  Lemma~\ref{lem:fmu-t} and~\ref{lem:compact-IL} with $\delta/2$. 
  If $y^+_{t}-f(\xbm_{t+1})\leq 0$, with probability greater than $1-\delta$, 
   \begin{equation} \label{eqn:compact-IL-instregret-pf-1}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t} - f(\xbm^*)  \leq I_t(\xbm^*) 
          \leq EI_t(\bar{\xbm}^*_t,\alpha)  + \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq&  EI_t^{\alpha}(\xbm_{t+1},\alpha)  + \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          =& (y^+_{t}-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1}),\alpha)+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))+  \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& (y^+_{t}-f(\xbm_{t+1})+f(\xbm_{t+1})-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1}),\alpha)+0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+  \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+ \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
  where the first line uses Lemma~\ref{lem:compact-IL}, the second line uses the definition of $\xbm_t$, and the last line uses Lemma~\ref{lem:fmu-t}, $\Phi(\cdot)<1$, and $y^+_{t}-f(\xbm_{t+1})\leq 0$.
 If $y^+_{t}-f(\xbm_{t+1})> 0$, with probability greater than $1-\delta$,
    \begin{equation} \label{eqn:compact-IL-instregret-pf-2}
  \centering
  \begin{aligned}
        r_t =& f(\xbm_{t+1})-f(\xbm^*) =  f(\xbm_{t+1})-y^+_{t}+ y^+_{t}-f(\xbm^*)\\
              \leq& f(\xbm_{t+1})-y^+_{t}+EI_{t}(\bar{\xbm}_{t}^*,\alpha) + \beta^{1/2}_t\sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
                =& f(\xbm_{t+1})-y^+_{t}+(y^+_{t}-f(\xbm_{t+1})+f(\xbm_{t+1})-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))\\
                  &+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))  + \beta^{1/2}_t\sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
               \leq&\beta_t^{1/2}\sigma_{t}(\xbm_{t+1}) +0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+ \beta^{1/2}_t\sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}. 
  \end{aligned}
  \end{equation}
  The first inequality in~\eqref{eqn:compact-IL-instregret-pf-2} is by Lemma~\ref{lem:compact-IL}, while the last inequality is due to Lemma~\ref{lem:fmu-t}, Lemma~\ref{lem:phi}, and $y^+_{t}-f(\xbm_{t+1})> 0$. 
   Combine~\eqref{eqn:compact-IL-instregret-pf-1} and~\eqref{eqn:compact-IL-instregret-pf-2} and the proof is complete.
\end{proof}
\begin{theorem}\label{thm:compact-regretbound-IL}
Given $\delta\in(0,0.698)$, let  $\beta_t = \max\{1,c_{\beta}^{-1}\log ( 2\pi_t c_{\alpha}/\delta)\} + c_{\beta}^{-1} \log(1+rt^2 L) $, where $\pi_t=\frac{\pi^2t^2}{6}$, $c_{\alpha} = 1.09$, and $c_{\beta}=0.427$.
The BO-EI Algorithm~\ref{} maintains the regret bound
 \begin{equation} \label{eqn:compact-regbound-IL-1}
  \centering
  \begin{aligned}
     P\left\{ R_T \leq \frac{1}{2} \beta_T^{1/2} ( C_{\gamma} T  \gamma_T)^{1/2}+0.4 \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}}+\sum_{t=1}^T \beta^{1/2}_t \sigma_{t}^{\alpha}(\xbm^*)+M_h+2\right\}  \geq 1-\delta,
  \end{aligned}
\end{equation}
for any $T$, where $C_{\gamma}=8/log(1+\sigma^{-2})$ and $M_h$ is some constant. 
\end{theorem}
\begin{proof}
   From Lemma~\ref{lem:variancebound} and Hölder's inequality, we know~\eqref{eqn:EI-insregret-pf-5} stands.
   From Lemma~\ref{lem:compact-IL-instregret} and the choice of $\beta_t$, we have~\eqref{eqn:compact-IL-instregret-1} with probability $\geq 1-\delta$.

   The posterior variance $\sigma_{t}(\xbm)$ is a Lipschitz continuous function of $\xbm$ and its Lipschitz constant, denoted as $L_{t}^{\sigma}$ is a function of $h_t$, $t$ and the kernel functions. In~\cite{lederer2019uniform} (Theorem 3.1), it is shown that $L_{t}^{\sigma}=\mathcal{O}(\frac{1}{\sqrt{t}})$ as $t\to\infty$ if $h_t=\mathcal{O}(\frac{1}{t^2})$, which is our choice in this section~\eqref{eqn:ht-1}. 
   From Lemma~\ref{lem:compact-IL-instregret}, with probability $\geq 1-\delta$, 
 \begin{equation} \label{eqn:compact-regbound-IL-pf-1}
  \centering
  \begin{aligned}
   r_t \leq&\beta_t^{1/2}\sigma_{t}(\xbm_{t+1}) +0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+ \beta^{1/2}_t (\sigma_{t}^{\alpha}(\xbm^*)+ L_{t}^{\sigma}(h_t) \norm{\bar{\xbm}^*_t-\xbm^*})+\frac{1}{t^2}\\
      \leq&\beta_t^{1/2}\sigma_{t}(\xbm_{t+1}) +0.4\sigma_{t}^{\alpha}(\xbm_{t+1})+ \beta^{1/2}_t \sigma_{t}^{\alpha}(\xbm^*)+ \beta^{1/2}_t L_{t}^{\sigma}(h_t) \frac{1}{L t^2}+\frac{1}{t^2}. 
   \end{aligned}
\end{equation}
   Clearly, $\sum_{t=1}^{\infty} \beta^{1/2}_t L_{t}^{\sigma}(h_t) \frac{1}{L t^2}<\infty$.
   Define constant $M_h$ so that $\sum_{t=1}^{\infty} \beta^{1/2}_t L_{t}^{\sigma}(h_t) \frac{1}{L t^2}<M_h$.
   From~\eqref{eqn:compact-regbound-IL-pf-1} and~\eqref{eqn:EI-insregret-pf-5}, with probability $\geq 1-\delta$
 \begin{equation} \label{eqn:compact-regbound-pf-2}
  \centering
  \begin{aligned}
      R_T \leq 0.4\left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}} + \frac{1}{2} (C_{\gamma}T\beta_T\gamma_T)^{1/2}+ \sum_{t=1}^T  \beta_t^{1/2}\sigma_{t}^{\alpha}(\xbm^*)+ M_h+2,
   \end{aligned}
\end{equation}
   where $C_{\gamma}=8/\log(1+\sigma^{-2})$.
\end{proof}
 Based on Theorem~\ref{thm:compact-regretbound-IL}, if $ \sum_{t=1}^T \beta_t^{1/2} \sigma_{t}^{\alpha}(\xbm^*)= o(T)$, BO-EI algorithm is a no-regret algorithm with probability $\geq 1-\delta$.


\begin{remark}\label{remark:relaxlipschitz}
From the cumulative regret bound perspective, the Lipschitz continuity of $f$ can be relaxed to stand with a high probability. The results in this section could be extended in a straightforward manner.
\end{remark}
\begin{remark}\label{remark:asytoreg}
We point out here the challenge for a cumulative regret bound result of BO-EI from the perspective of the asymptotic convergence results. 
The asymptotic results cannot be extended to the cumulative regret bound analysis mainly due to the difficulty in establishing lower bounds for $y^+_{t}-\mu_{t}(\xbm^*)$ for all $t$. Since the sum of $r_t$ is considered, the probability of $1-\sqrt{\frac{\pi}{2}}$ tends to $0$  for all $t$ as $t\to\infty$. Using $\beta_t$ in place of $w$ in the analysis of Theorem~\ref{theorem:EI-convg-star} would make the lower bound of $y^+_{t}-\mu_{t}(\xbm^*)$ tend to $-\infty$ and hence the exploration and exploitation properties of EI can no longer be used. 
The ratio $\frac{\tau(\beta_t^{1/2})}{\tau(-\beta_t^{1/2})}$ in Theorem~\ref{theorem:EI-convergence-1} would increase $\to\infty$ quickly with $\beta_t$ as well.

Nevertheless, one might be more interested in finding a good approximation of $f(\xbm^*)$ than obtaining a no-regret optimization path, as~\cite{bull2011convergence} argues. As mentioned in the introduction, some authors have tried to achieve a theoretically-guaranteed reduction of $\sigma_{t-1}(\xbm^*)$ via aggressive sampling~\cite{hu2022adjustedeiregret}, or unbounded algorithmic parameters~\cite{tran2022regret}. 
Such algorithms however, might not be practical.  
\end{remark}
 


==> Sections/Vei.tex <==
\section{Variance expected improvement}\label{se:algorithm}
From the convergence analysis, it is clear that EI has strong asymptotoic convergence properties for a large number of functions.
However, its fixed trade-off between exploitation and exploration determined by the nonconvex EI function might not generate a no-regret algorithm. 
In this section, we propose a simple modification to achieve the no-regret properties that might be more preferrable for some applications, as well as improved probability for the asymptotic convergence result. We first point out  that the theoretical bounds are often much larger than actual BO-EI results in practice. Therefore, the proposed algorithm, while enjoying improvement theoretical properties, is not guaranteed for better performance in practice. 

The variance $\sigma_{t}(\xbm^*)$ at the optimal point $\xbm^*$ is one of the main difficulty in our analysis. Therefore, we add an explicit expression of $\sigma_t(\xbm)$ to EI so that exploration is guaranteed to be emphasized as the iteration progresses, which then ensures $\sigma_{t}(\xbm)$ is reduced at any $\xbm\in C$, including $\xbm^*$. 
The modified EI with enhanced exploration is referred to as variance expected improvement (VEI) with the following expression
\begin{equation} \label{eqn:VEI}
 \centering
  \begin{aligned}
       VEI_t(\xbm,\alpha) =   (y_{t}^+-\mu_{t}(\xbm))\Phi(z_{t}(\xbm,\alpha))+\sigma_{t}^{\alpha}(\xbm)\phi(z_{t}(\xbm,\alpha))+\theta \sigma_{t}^{\alpha}(\xbm), 
  \end{aligned}
\end{equation}
where $\alpha\in (0,1]$ and $z_{t}(\xbm,\alpha) = \frac{y_{t}^+-\mu_{t}(\xbm)}{\sigma_{t}^{\alpha}(\xbm)}$.
The explicit standard deviation terms resembles that of UCB. 
We state the convergence theorems for VEI under the GP prior assumptions.
\subsection{VEI under GP prior assumption}\label{se:vei-gp}
In this section, Assumption~\ref{assp:gp} and~\ref{assp:constraint} are valid.
\begin{theorem}\label{theorem:VEI-convg}
   Given $\delta\in(0,1)$, let $\beta=\max\{1, c_{\beta}^{-1} \log (2c_{\alpha}/\delta)\}$ and $\theta\geq \beta^{1/2}$.
   Runing the BO-VEI algorithm with GP prior $(0,k(\xbm,\xbm'))$ leads to the convergence rate 
      \begin{equation} \label{eqn:VEI-convg-star-1}
  \centering
  \begin{aligned}
      r_t  \leq  (2M+2c_\sigma\sigma)\frac{3}{t}+ (0.4+\beta^{1/2}+\theta) \sigma_{t_k}^{\alpha}(\xbm_{t_k+1}))\}, 
   \end{aligned}
  \end{equation} 
  with probability $\geq 1-(\frac{1}{2})^{t/3}-2\Phi(-c_{\sigma})-\delta$.
\end{theorem}
\begin{proof}
   Similar to Theorem~\ref{theorem:EI-convg-star}, we know that with probability $1-2\Phi(-c_{\sigma})$,
  \begin{equation} \label{eqn:VEI-convg-star-pf-1}
  \centering
  \begin{aligned}
        \sum_{t=0}^{T-1}  y^+_{t}-y^+_{t+1} \leq y^+_0 - y_T^+ \leq 2 M +2c_{\sigma}\sigma. 
  \end{aligned}
  \end{equation}
  Therefore, $y^+_{t}-y^+_{t+1} \geq \frac{2M +2c_{\sigma}\sigma}{k}$ at most $k$ times for any $k\in \Nbb$. 
  Let $k=[t/2]$ so that $2k\leq t\leq 2(k+1)$.
  There exists time $k\leq t_k\leq 2k$ so that $y^+_{t_k}-y^+_{t_k+1} < \frac{2M +2c_{\sigma}\sigma}{k}$. 
   Consider first the noiseless case $\sigma=0$.   

  The choice of $\beta$ satisfies Lemma~\ref{lem:IEIbound} and Lemma~\ref{lem:fmu} with $\delta/2$.
  From Lemma~\ref{lem:IEIbound} and $\theta\geq \beta^{1/2}$, with probability $\geq 1-\delta/2$,
  \begin{equation} \label{eqn:VEI-convg-star-pf-2}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t}-f(\xbm^*)\leq y^+_{t_k-1}-f(\xbm^*) = I_{t_k}(\xbm^*)\\
               \leq& EI_{t_k}(\xbm^*,\alpha) + \beta^{1/2}\sigma_{t_k}^{\alpha}(\xbm^*)
               \leq EI_{t_k}(\xbm^*,\alpha) + \theta\sigma_{t_k}^{\alpha}(\xbm^*)
               \leq EI_{t_k}(\xbm_{t_k+1},\alpha) + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\\
                =& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+\sigma_{t_k}^{\alpha}(\xbm_{t_k+1})\phi(z_{t_k}(\xbm_{t_k+1},\alpha))  + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).\\
             \leq& (y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}))\Phi(z_{t_k}(\xbm_{t_k+1},\alpha))+0.4\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) + \theta\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).
   \end{aligned}
  \end{equation}
    From Lemma~\ref{lem:fmu}, with probability $\geq 1-\delta/2$, 
   \begin{equation} \label{eqn:VEI-convg-star-pf-3}
  \centering
  \begin{aligned}
          y^+_{t_k}-\mu_{t_k}(\xbm_{t_k+1}) = y^+_{t_k}-f(\xbm_{t_k+1})+f(\xbm_{t_k+1})-\mu_{t_k}(\xbm_{t_k+1}) \leq \frac{2M}{k} +\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1}).
    \end{aligned}
  \end{equation}
  Applying~\eqref{eqn:VEI-convg-star-pf-3} to~\eqref{eqn:VEI-convg-star-pf-2}, we have with probability $\geq 1-\delta$, 
  \begin{equation} \label{eqn:VEI-convg-star-pf-6}
  \centering
  \begin{aligned}
          r_t  \leq& \frac{2M}{k}+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})+(0.4+\theta)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}).\\
  \end{aligned}
  \end{equation}

   Next, we consider the noisy case using similar technique as in Theorem~\ref{theorem:EI-convergence-1}. Given a sequence of iterates $\xbm_i$  of size $k\in \Nbb$ where $i\in A_k$, \textit{i.e.}, $|A_k|=k$, the probability of $f(\xbm_i) < y_i = f(\xbm_i)+\epsilon(\xbm_i)$ for all $i\in A_k$ is $(\frac{1}{2})^k$.
   Let $k=[t/3]$ so that $3k\leq t\leq 3(k+1)$.
   There exists $k \leq t_k \leq 3k$ so that $y_{t_k}^+-y_{t_k+1}^+<\frac{2M_f+2c_{\sigma}\sigma}{k}$ and $f(\xbm_{t_k+1})\geq y_{t_k+1}\geq y_{t_k+1}^+$ with probability $\geq 1-(\frac{1}{2})^k$.
 Following the same analysis for the noiseless case   
  with probability $\geq 1-(\frac{1}{2})^k-\delta-2\Phi(-c_{\sigma})$, 
  \begin{equation} \label{eqn:VEI-convg-star-pf-7}
  \centering
  \begin{aligned}
         r_t  \leq& \frac{2M+2c_{\sigma}\sigma}{k}+\beta^{1/2}\sigma_{t_k}(\xbm_{t_k+1})+(0.4+ \theta)\sigma_{t_k}^{\alpha}(\xbm_{t_k+1}) .\\
  \end{aligned}
  \end{equation}
  The proof is complete.
\end{proof}

In addition, BO-VEI can be shown to be a no-regret algorithm with our definition of $r_t$.
For brevity of presentation, we use the same discretization $\Cbb_t$ for compact $C$ as in Section~\ref{se:compact}. 
\begin{theorem}\label{thm:VEI-regret}
Given $\delta\in(0,0.698)$, let  $\beta_t = \max\{1,c_{\beta}^{-1}\log ( 2\pi_t c_{\alpha}/\delta)\} + c_{\beta}^{-1} \log(1+rt^2 L) $, where $\pi_t=\frac{\pi^2t^2}{6}$, $c_{\alpha} = 1.09$, and $c_{\beta}=0.427$.
The BO-VEI Algorithm~\ref{} maintains the regret bound
 \begin{equation} \label{eqn:VEI-regbound-1}
  \centering
  \begin{aligned}
     P\left\{ R_T \leq \frac{1}{2} \beta_T^{1/2} ( C_{\gamma} T  \gamma_T)^{1/2}+0.4 \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}}+2\right\}  \geq 1-\delta,
  \end{aligned}
\end{equation}
for any $T$, where $C_{\gamma}=8/log(1+\sigma^{-2})$. 
\end{theorem}
\begin{proof}
   Notice that the $\beta_t$ in this theorem satisfies the conditions in both  Lemma~\ref{lem:fmu-t} and~\ref{lem:compact-IL} with $\delta/2$. 
  If $y^+_{t}-f(\xbm_{t+1})\leq 0$, with probability greater than $1-\delta$, 
   \begin{equation} \label{eqn:VEI-regbound-pf-1}
  \centering
  \begin{aligned}
          r_t  =& y^+_{t} - f(\xbm^*)  \leq I_t(\xbm^*) 
          \leq EI_t(\bar{\xbm}^*_t,\alpha)  + \beta_t^{1/2} \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\ 
          \leq& EI_t(\bar{\xbm}^*_t,\alpha)  + \theta \sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}
          \leq  EI_t^{\alpha}(\xbm_{t+1},\alpha)  + \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\ 
          =& (y^+_{t}-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm),\alpha)+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_t,\alpha))+  \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\ 
          \leq& \beta_t^{1/2}\sigma_{t}(\xbm_{t+1})+(0.4+\theta)\sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
  where the first line uses Lemma~\ref{lem:compact-IL}, the second line uses the definition of $\xbm_t$, and the last line uses Lemma~\ref{lem:fmu-t}.
   If $y^+_{t}-f(\xbm_{t+1})> 0$, with probability greater than $1-\delta$,
    \begin{equation} \label{eqn:VEI-regbound-pf-2}
  \centering
  \begin{aligned}
        r_t =& f(\xbm_{t+1})-f(\xbm^*) =  f(\xbm_{t+1})-y^+_{t}+ y^+_{t}-f(\xbm^*)\\
              \leq& f(\xbm_{t+1})-y^+_{t}+EI_{t}(\bar{\xbm}_{t}^*,\alpha) + \beta^{1/2}_t\sigma_{t}^{\alpha}(\bar{\xbm}^*_t)+\frac{1}{t^2}\\
                \leq& f(\xbm_{t+1})-y^+_{t}+(y^+_{t}-f(\xbm_{t+1})+f(\xbm_{t+1})-\mu_{t}(\xbm_{t+1}))\Phi(z_{t}(\xbm_{t+1},\alpha))\\
                  &+\sigma_{t}^{\alpha}(\xbm_{t+1})\phi(z_{t}(\xbm_{t+1},\alpha))  + \theta \sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}\\
               \leq&\beta_t^{1/2}\sigma_{t}(\xbm_{t+1}) +(0.4+\theta)\sigma_{t}^{\alpha}(\xbm_{t+1})+\frac{1}{t^2}, 
  \end{aligned}
  \end{equation}
where the second line uses Lemma~\ref{lem:compact-IL}, the third line uses the definition of $\xbm_{t+1}$, and the last line uses Lemma~\ref{lem:fmu-t}. 


  From Lemma~\ref{lem:variancebound} and Hölder's inequality,~\eqref{eqn:EI-insregret-pf-5} stands.
   Thus, with probability $\geq 1-\delta$
 \begin{equation} \label{eqn:VEI-regbound-pf-3}
  \centering
  \begin{aligned}
      R_T =\sum_{t=1}^Tr_t  \leq (0.4+\theta) \left(\frac{1}{4}C_{\gamma}\gamma_T\right)^{\frac{\alpha}{2}} T^{\frac{1+1-\alpha}{2}} + \frac{1}{2} (C_{\gamma}T\beta_T\gamma_T)^{1/2}+2,
   \end{aligned}
\end{equation}
   where $C_{\gamma}=8/\log(1+\sigma^{-2})$.
\end{proof}
For commonly used kernels such as squared exponential functions~\cite{srinivas2009gaussian}, BO-VEI algorithm is a no-regret algorithm.

\subsection{VEI under RKHS assumption}\label{se:vei-gp-rkhs}

